Multi Target Tracking by Learning from Generalized Graph Differences

Formulating the multi object tracking problem as a network flow optimization problem is a popular choice. In this paper an efficient way of learning the weights of such a network is presented. It separates the problem into one embedding of feasible solutions into a one dimensional feature space and one optimization problem. The embedding can be learned using standard SGD type optimization without relying on an additional optimizations within each step. Training data is produced by performing small perturbations of ground truth tracks and representing them using generalized graph differences, which is an efficient way introduced to represent the difference between two graphs. The proposed method is evaluated on DukeMTMCT with competitive results.

==> table_with_graphs.tex <==

\begin{table}
\small

\begin{center}
\centering
\begin{tabular}{@{}ccc@{}}
\toprule
Name & Ground Truth & Possible Error \\
\midrule
\\
\makecell{ID\\Switch}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node[draw,circle] (B) at (1,0) {$ $};
\node[draw,circle] (C) at (0,1) {$ $};
\node[draw,circle] (D) at (1,1) {$ $};
\draw[->] (A) -> (B);
\draw[->] (C) -> (D);
\end{tikzpicture}
\end{tabular}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node[draw,circle] (B) at (1,0) {$ $};
\node[draw,circle] (C) at (0,1) {$ $};
\node[draw,circle] (D) at (1,1) {$ $};
\draw[->] (A) -> (D);
\draw[->] (C) -> (B);
\end{tikzpicture}
\end{tabular}
\\
%\hline



\\
Split
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node[draw,circle](C) at (1,0) {$ $};
\path[->,draw,thick]
    (A) edge node {$$} (C)  ;
\end{tikzpicture}
\end{tabular}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node (B) at (0.5,0.5) {$ $};
\node[draw,circle](C) at (1,0) {$ $};
\path[->,draw,thick]
    (A) edge [bend right=20]  node {$$} (B)  ;
\path[->,draw,thick]
    (B) edge [bend right=20]  node {$$} (C)  ;
\end{tikzpicture}
\end{tabular}
\\
%\hline

\\
Merge
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node (B) at (0.5,0.5) {$ $};
\node[draw,circle](C) at (1,0) {$ $};
\path[->,draw,thick]
    (A) edge [bend right=20]  node {$$} (B)  ;
\path[->,draw,thick]
    (B) edge [bend right=20]  node {$$} (C)  ;
\end{tikzpicture}
\end{tabular}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node[draw,circle](C) at (1,0) {$ $};
\path[->,draw,thick]
    (A) edge node {$$} (C)  ;
\end{tikzpicture}
\end{tabular}
\\
%\hline

\\
\makecell{Split\\and\\Merge}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node[draw,circle](B) at (1,0) {$ $};
\node[draw,circle](C) at (1,-1) {$ $};
\node (D) at (0.5,0.5) {$ $};
\path[->,draw,thick]
    (D) edge [bend right=20]  node {$$} (C)  ;
\path[->,draw,thick]
    (A) edge node {$$} (B)  ;
\end{tikzpicture}
\end{tabular}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node[draw,circle](B) at (1,0) {$ $};
\node[draw,circle](C) at (1,-1) {$ $};
\node (D) at (0.5,0.5) {$ $};
\path[->,draw,thick]
    (D) edge [bend right=20]  node {$$} (B)  ;
\path[->,draw,thick]
    (A) edge node {$$} (C)  ;
\end{tikzpicture}
\end{tabular}
\\
%\hline

\\
\makecell{Double\\Split\\and\\Merge}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node (AA) at (0.5,-0.5) {$ $};
\node[draw,circle] (B) at (1,0) {$ $};
\node[draw,circle] (C) at (0,1) {$ $};
\node[draw,circle] (D) at (1,1) {$ $};
\node (DD) at (0.5,1.5) {$ $};
\draw[->] (A) -> (B);
\draw[->] (C) -> (D);
\end{tikzpicture}
\end{tabular}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node (AA) at (0.5,-0.5) {$ $};
\node[draw,circle] (B) at (1,0) {$ $};
\node[draw,circle] (C) at (0,1) {$ $};
\node[draw,circle] (D) at (1,1) {$ $};
\node (DD) at (0.5,1.5) {$ $};
\draw[->] (C) -> (B);
\path[->,draw,thick]
    (A) edge [bend left=20] node {$$} (AA)  ;
\path[->,draw,thick]
    (DD) edge [bend right=20] node {$$} (D)  ;
\end{tikzpicture}
\end{tabular}
\\
%\hline
\bottomrule
\end{tabular}
\end{center}
\normalsize
\caption{Switch, split and merge errors introduced to form training data pairs from ground truth.}
\label{tab:subgraphs}
\end{table}

\begin{table}
\small
\begin{center}
\centering
\begin{tabular}{@{}ccc@{}}
\toprule
 Name & Ground Truth & Possible Error \\
\midrule

\\
\makecell{Detection\\Skip}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node[draw,circle] (B) at (1,0) {$ $};
\node[draw,circle] (C) at (2,0) {$ $};
\path[->,draw,thick]
    (A) edge node {$$} (B)  ;
\path[->,draw,thick]
    (B) edge node {$$} (C)  ;
\end{tikzpicture}
\end{tabular}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node[draw,circle] (B) at (1,0) {$ $};
\node[draw,circle] (C) at (2,0) {$ $};
\path[->,draw,thick]
    (A) edge [bend left=30]  node {$$} (C)  ;
\end{tikzpicture}
\end{tabular}
\\
%\hline

\\
\makecell{Skip\\First}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node (B) at (-0.5,0.5) {$ $};
\node[draw,circle] (C) at (1,0) {$ $};
\path[->,draw,thick]
    (B) edge [bend right=20] node {$$} (A)  ;
\draw[->] (A) -> (C);
\end{tikzpicture}
\end{tabular}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node (B) at (0.5,0.5) {$ $};
\node[draw,circle] (C) at (1,0) {$ $};
\path[->,draw,thick]
    (B) edge [bend right=20] node {$$} (C)  ;
\end{tikzpicture}
\end{tabular}
\\
%\hline

\\
\makecell{Skip\\Last}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node (B) at (1.5,-0.5) {$ $};
\node (D) at (1.5,0.5) {$ $};
\node[draw,circle] (C) at (1,0) {$ $};
\path[->,draw,thick]
    (C) edge [bend left=20] node {$$} (B)  ;
\draw[->] (A) -> (C);
\end{tikzpicture}
\end{tabular}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node (B) at (0.5,0.5) {$ $};
\node (D) at (0.5,-0.5) {$ $};
\node[draw,circle] (C) at (1,0) {$ $};
\path[->,draw,thick]
    (A) edge [bend left=20] node {$$} (D)  ;
\end{tikzpicture}
\end{tabular}
\\
%\hline

\\
\makecell{Extra\\First}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node (B) at (0.5,-0.5) {$ $};
\node (D) at (0.5,0.5) {$ $};
\node[draw,circle] (C) at (1,0) {$ $};
\path[->,draw,thick]
    (D) edge [bend right=20] node {$$} (C)  ;
\end{tikzpicture}
\end{tabular}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node (B) at (-0.5,0.5) {$ $};
\node (D) at (-0.5,-0.5) {$ $};
\node[draw,circle] (C) at (1,0) {$ $};
\path[->,draw,thick]
    (B) edge [bend right=20] node {$$} (A)  ;
\draw[->] (A) -> (C);
\end{tikzpicture}
\end{tabular}
\\
%\hline


\\
\makecell{Extra\\Last}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node[draw,circle] (B) at (1,0) {$ $};
\node (C) at (0.5,-0.5) {$ $};
\path[->,draw,thick]
    (A) edge [bend right=20]  node {$$} (C)  ;
\end{tikzpicture}
\end{tabular}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node[draw,circle] (B) at (1,0) {$ $};
\node (C) at (1.5,-0.5) {$ $};
\path[->,draw,thick]
    (A) edge  node {$$} (B)  ;
\path[->,draw,thick]
    (B) edge [bend right=20] node {$$} (C)  ;
\end{tikzpicture}
\end{tabular}
\\
%\hline
\bottomrule

\end{tabular}
\end{center}
\normalsize
\caption{Skip and extra errors introduced to form training data pairs from ground truth.}
\label{tab:subgraphs2}
\end{table}

\begin{table}
\small
\begin{center}
\centering
\begin{tabular}{@{}ccc@{}}
\toprule
Name & Ground Truth & Possible Error \\
\midrule
\\
\makecell{False\\positive}
&
\begin{tabular}{c}
\begin{tikzpicture}
\end{tikzpicture}
\end{tabular}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node (A) at (0,0) {$ $};
\node[draw,circle,dashed] (B) at (0.5,-0.5) {$ $};
\node(C) at (1,0) {$ $};
\path[->,draw,thick]
    (A) edge [bend right=20]  node {$$} (B)  ;
\path[->,draw,thick]
    (B) edge [bend right=20]  node {$$} (C)  ;
\end{tikzpicture}
\end{tabular}
\\
%\hline

\\
\makecell{Split\\to\\False\\ Positive}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node[draw,circle] (B) at (1,0) {$ $};
\node[draw,circle] (C) at (2,0) {$ $};
\node[draw,circle,dashed] (D) at (2,-1) {$ $};
\node (E) at (1.5,0.5) {$ $};
\node (F) at (2.5,-1.5) {$ $};
\path[->,draw,thick]
    (A) edge  node {$$} (B)  ;
\path[->,draw,thick]
    (B) edge  node {$$} (C)  ;
\end{tikzpicture}
\end{tabular}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node[draw,circle] (B) at (1,0) {$ $};
\node[draw,circle] (C) at (2,0) {$ $};
\node[draw,circle,dashed] (D) at (2,-1) {$ $};
\node (E) at (1.5,0.5) {$ $};
\node (F) at (2.5,-1.5) {$ $};
\path[->,draw,thick]
    (A) edge  node {$$} (B)  ;
\path[->,draw,thick]
    (B) edge  node {$$} (D)  ;
\path[->,draw,thick]
    (E) edge [bend right=20] node {$$} (C)  ;
\path[->,draw,thick]
    (D) edge [bend right=20] node {$$} (F)  ;
\end{tikzpicture}
\end{tabular}
\\
%\hline

\\
\makecell{Split\\from\\False\\ Positive}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node[draw,circle] (B) at (1,0) {$ $};
\node[draw,circle] (C) at (2,0) {$ $};
\node[draw,circle,dashed] (D) at (1,-1) {$ $};
\node (E) at (1.5,0.5) {$ $};
\node (F) at (2.5,-1.5) {$ $};
\path[->,draw,thick]
    (A) edge  node {$$} (B)  ;
\path[->,draw,thick]
    (B) edge  node {$$} (C)  ;
\end{tikzpicture}
\end{tabular}
&
\begin{tabular}{c}
\begin{tikzpicture}
\node[draw,circle] (A) at (0,0) {$ $};
\node[draw,circle] (B) at (1,0) {$ $};
\node[draw,circle] (C) at (2,0) {$ $};
\node[draw,circle,dashed] (D) at (1,-1) {$ $};
\node (E) at (1.5,0.5) {$ $};
\node (F) at (0.5,-1.5) {$ $};
\path[->,draw,thick]
    (A) edge  node {$$} (B)  ;
\path[->,draw,thick]
    (B)  edge [bend right=20]  node {$$} (E)  ;
\path[->,draw,thick]
    (F) edge [bend left=20] node {$$} (D)  ;
\path[->,draw,thick]
    (D) edge node {$$} (C)  ;
\end{tikzpicture}
\end{tabular}
\\
%\hline
\bottomrule

\end{tabular}
\end{center}
\normalsize
\caption{False positives introduced to form training data pairs from ground truth.}
\label{tab:subgraphs3}
\end{table}
%-------------------

\begin{table}
\small
\begin{center}
\centering
\begin{tabular}{ccc}
\toprule
Name & Ground Truth & Possible Error \\
\midrule

\\
\makecell{Too Short\\Track}
&
\begin{tabular}{c}
\begin{tikzpicture}
\end{tikzpicture}
\end{tabular}
&
\begin{tabular}{c}
\begin{tikzpicture}[scale=0.75]
\node[draw,circle] (A) at (0,0) {$ $};
\node[draw,circle] (B) at (1,0) {$ $};
\node[draw,circle] (C) at (2,0) {$ $};
\node (D) at (1.5,0) {$\ldots$};
\node (E) at (-0.5,0.5) {$ $};
\node (F) at (2.5,0.5) {$ $};
\path[->,draw,thick]
    (A) edge  node {$$} (B)  ;

\path[->,draw,thick]
    (E) edge [bend right=20] node {$$} (A)  ;
\path[->,draw,thick]
    (C) edge [bend right=20] node {$$} (F)  ;

    %https://tex.stackexchange.com/questions/20885/draw-curly-braces-in-tikz
\draw [decorate,decoration={brace,mirror,amplitude=10pt}]
(-0.1,-0.2) -- (2.1,-0.2) node [black,midway,yshift=-17pt] {\footnotesize
$\frac{n_{\text{minlen}}}{2}$};
\end{tikzpicture}
\end{tabular}
\\
%\hline

\\
\makecell{Proper\\Track}
&
\begin{tabular}{c}
\begin{tikzpicture}[scale=0.75]
\node[draw,circle] (A) at (0,0) {$ $};
\node[draw,circle] (B) at (1,0) {$ $};
\node[draw,circle] (C) at (2,0) {$ $};
\node (D) at (1.5,0) {$\ldots$};
\node (E) at (-0.5,0.5) {$ $};
\node (F) at (2.5,0.5) {$ $};
\path[->,draw,thick]
    (A) edge  node {$$} (B)  ;

\path[->,draw,thick]
    (E) edge [bend right=20] node {$$} (A)  ;
\path[->,draw,thick]
    (C) edge [bend right=20] node {$$} (F)  ;
    
    %https://tex.stackexchange.com/questions/20885/draw-curly-braces-in-tikz
\draw [decorate,decoration={brace,mirror,amplitude=10pt}]
(-0.1,-0.2) -- (2.1,-0.2) node [black,midway,yshift=-17pt] {\footnotesize
$n_{\text{minlen}}$};
\end{tikzpicture}
\end{tabular}
&
\begin{tabular}{c}
\begin{tikzpicture}
\end{tikzpicture}
\end{tabular}
\\
\bottomrule
\end{tabular}
\end{center}
\normalsize
\caption{Track lengths data pairs used for training.}
\label{tab:subgraphs4}
\end{table} 
